A Pre-defined Sparse Kernel Based Convolution for Deep CNNs

The high demand for computational and storage resources severely impede the deployment of deep convolutional neural networks (CNNs) in limited-resource devices. Recent CNN architectures have proposed reduced complexity versions (e.g. SuffleNet and MobileNet) but at the cost of modest decreases inaccuracy. This paper proposes pSConv, a pre-defined sparse 2D kernel-based convolution, which promises significant improvements in the trade-off between complexity and accuracy for both CNN training and inference. To explore the potential of this approach, we have experimented with two widely accepted datasets, CIFAR-10 and Tiny ImageNet, in sparse variants of both the ResNet18 and VGG16 architectures. Our approach shows a parameter count reduction of up to 4.24x with modest degradation in classification accuracy relative to that of standard CNNs. Our approach outperforms a popular variant of ShuffleNet using a variant of ResNet18 with pSConv having 3x3 kernels with only four of nine elements not fixed at zero. In particular, the parameter count is reduced by 1.7x for CIFAR-10 and 2.29x for Tiny ImageNet with an increased accuracy of ~4%.

==> Allerton pSConv 2019/sec_psconv.tex <==

We now describe pSConv, our proposed approach to reduce the number of parameters in convolutional neural networks via pre-defined sparse kernels. In pSConv, we exploit the structural sparsity of the input receptive-field (RF) \cite{brendel2019approximating} and propose pre-defined sparse 2D kernel based CONVs to form the channels of each convolutional layer.

% In prior works, exploitation of sparsity of the filter kernels across IFM channels have shown promising results. Also, \cite{dey2019pre} has shown pre-defined sparsity based fully connected (FC) layers provide large amount of weight reduction at the cost of nominal accuracy drop for MLPs. 

\subsection{Pre-Defined Sparse CONV Filters}
\label{sub:psconv}
Assume a convolutional layer $L$ with $C$ CONV filters where each filter is of dimension $k \times k \times C_i^L$ (here, $H_{f}^L$ = $W_{f}^L$ = $k$).\footnote{Typically, $k\in\{1, 3, 5, 7\}$ in modern convolutional neural networks.}  We define a $k \times k \times C_i^L$ pre-defined sparse CONV filter as  one in which some of the $k^2 C_i^L$ elements are fixed to be zero and this pattern is fixed before training and held fixed throughout training and inference. A {\em regular} pre-defined sparse CONV filter has the same kernel support size  for each 2D kernel that comprises the CONV filter. Here, the {\em kernel support size} (KSS), $y\in \{1,\ldots,k^2\}$, is defined to be the number of non-zero weight entries in each $k\times k$ 2D kernel of the CONV filter.\footnote{The kernel support is the set of indices where the kernel is not constrained to be zero.} For example, Fig. \ref{fig:pSConv_kernel}(a) and (b) illustrate instances of kernels with KSS of 4 and 3, respectively. 
% PAB: THis sentence seems out of place to me and has confusing terminology...
The specific method for designing the patterns of kernel support (i.e., constrained zero element patterns) in the CONV filter may vary with implications discussed briefly below.

\begin{figure}[h!]
\includegraphics[width=0.7\linewidth]{Figs/Sparse_2D_kernel.png}
\centering
\caption{Kernel structure of pre-defined sparse 2D kernels with KS of (a) 4, and (b) 3, respectively. Here $W_{(p)ij}^{(l,m)}$ signifies the $(i,j)^{th}$ element of $p^{th}$ 2D kernel of $m^{th}$ filter in layer $l$.}
\label{fig:pSConv_kernel}
\end{figure}

\iffalse
%%%%%%%%%%%%%keith's suggestions%%%%%%%%%%%%%%%%%

1) A $k \times k \times C_H^L$ pre-defined sparse CONV filter is one where some of the $k^2 C_H^L$ elements are fixed to be zero and this pattern is fixed before training and held fixed throughout training and inference.
2) A regular, pre-defined sparse CONV filter have the same KS for each 2D kernel that comprises the CONV filter.   Here, the support is defined to be the number of ...

3) The specific method for designing the pattern of non-zeros in the CONV filter may vary.

4) All of the results presented in this paper are generated using  regular sparse CONV filters wherein the KS were selected in a constrained, pseudo-random manner.  The constraint enforced is that at least one $C_H^L$ 2D kernels must be non-zero for each of the $k^2$ locations. 
%%%SK: change non-zero terms to KS, as and when needed. add : one of the $C_H^(L) ...$. Change all 2D as kernel and 3D as filter...

3) A regular, pre-defined sparse $k \times k \times C_H^L$ CONV filter has the same number of non-zero elements for each channel 2D filter. 
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
For example, for $k=3$, there are $9$ possible values of $y$, with $y=9$ denoting the standard 2D kernel without any pre-defined sparsity, and $y=4$ denotes that only four non-zero entries are allowed in the $3 \times 3$ kernel space while the remaining five entries are $0$. Furthermore, for a given KSS, the pattern of non-zero entries is \textit{pre-defined} at the start of the training process. All results presented in this paper were generated using regular pre-defined sparse CONV filters wherein the kernel support (i.e., patterns of defining the sparsity)  were selected in a constrained, pseudo-random manner. The constraint  enforced  ensured that at least one of the $C_i^L$ 2D kernels has non-zero element for each of the $k^2$ locations. Thus, this procedure provides patterns for sparse CONV layers with significantly fewer parameters,  while the receptive field of the CONV filter remains $k \times k$.
The pSConv concept is illustrated in  Fig. \ref{fig:pSConv} where $C$  regular pre-defined sparse CONV filters using a KSS of 4 (i.e., 5 zero locations in each $3\times 3$ kernel) map an IFM of dimension $H_i^L \times W_i^L \times C_i^L$ to an OFM of dimension $H_o^L \times W_o^L \times C_o^L$.  

\subsection{Training for pSConv}

Pre-defined sparsity in CONV filters has the potential to reduce storage and computation complexity, both during training and inference. Storage may be reduced since only the potentially nonzero elements need to be stored, for instance, with a KSS of 3 for a $3\times 3$ 2D kernel, only $(1/3)^{rd}$ of the weights need to be stored. During the forward processing, only the KSS weights need to be multiplied with the input feature maps. Furthermore, during back-propagation of training, the gradient flow only needs to pass through the kernel support. Realizing these potential complexity reductions in practice, however, requires careful design of the kernel support patterns and the associated memory and computational resources. In software, for example, the storage and computation demands for linked-list storage and the associated array referencing may eliminate a significant fraction of these advantages  associated with sparsity. Similar issues will arise in custom hardware acceleration. However these challenges can be alleviated by designing kernel support patterns algorithmically with a small complexity overhead. 
For example, a very similar problem was solved in \cite{dey2019pre} where it was also shown that these structured connection patterns typically outperformed randomly generated patterns.  Another approach is to utilize more generic sparse tensor product accelerators that may be available in hardware or software libraries \cite{han2016eie}. However, this paper focuses on assessing the potential efficacy of pSConv layers and therefore we do not address the above issues.   Specifically, our implementations targeted rapid software development for experimentation and did not attempt to optimize the complexity for sparsity. 
\iffalse
*** Ideally, an optimized implementation in SW/HW.  

1) Using pre-defined sparity in CONV filters can reduce both the storage and computational complexity (FLOPs) of the network.  

2) Storage may be reduced since only the non-zero weights need be stored -- e.g., with a KS of 3 for a $3\times 3$ 2D kernel, there are 1/3 of the weights to store.  

3) Computational complexity may also be reduced since the in the forward processing only the weights in the kernel support need to be multiplied with the input features.  Furthermore, in the back-propagation during training the gradient flow need only pass through the KS.  

4) realizing these potential complexity reductions in practice, however, requires careful design of the KS patterns and the associated memory and computational resources. 

5) In software, for example, the storage and computation demands for linked-list storage and the associated array referencing may eliminate much of the above advantages  associated with sparsity.  

6) Similar issues will arise in custom hardware acceleration.  However, these challenges may be addressed by designing KS patterns that are algorithmically generated.  This eliminates the need to store the KS pattern and, if the algorithm is simple enough, the associated computational complexity will be a small fraction of the savings associated with sparsity.  Such a design has been developed for fully-connected layers in \cite{dey2018highly} where it was also shown that the added constraints to the support patterns did not degrade performance.  Similar approaches may be extended to software implementations.

6b) Another approach is to utilize more generic sparse tensor product accelerators that may be available in hardware or software libraries. \cite{han2016eie}.  

7) However, this paper focuses on assessing the efficacy of pSConv layers and therefore our experiments in this paper do not attempt to address the above issues.   Specifically, our implementation targeted rapid software development for experimentation and did not attempt to optimize the complexity for sparsity.   

8) Our specific implementation used Pytorch and we simply zeroed out the weights in the locations outside of the KS at the start of training and at the end of each batch -- i.e., weights were initially updated without a sparsity assumption and then reset to zero before the next batch.  
%SK: \cite{han2016eie} after mentioning dedicated hardware or software packages to support adv of sparse matrix mult.
***   
\fi

Our specific implementation used Pytorch as development package and we zeroed out the weights in the locations outside of kernel support  at the start of training and at the end of each mini-batch update -- i.e., the  weights were initially updated without a sparsity assumption and then those outside the kernel support we reset to zero before the next mini-batch. 

% Consider a CONV filter based weight tensor $W^{(L)}$ with size $C \times k \times k \times C_H^L$ with $C$ denoting the number of output channels, and $L$ denoting the layer index. Let $\alpha^{(L)}$ denote the tensor with size $C \times k \times k \times C_H^L$, i.e. the size of the CONV tensor $W^{(L)}$. The entries in $\alpha^{(L)}$ can be either 0 or 1. The locations of zeros and ones in $\alpha^{(L)}$ capture the pre-defined sparsity pattern of CONV $W^{(L)}$. Specifically, for the locations in which $W^{(L)}$ is zero, the entries in $\alpha^{(L)}$ are also 0, while for the remaining locations, $\alpha^{(L)}$ is set to 1. 

% At the start of training, let $W_{\text{init}}^{(L)}$ denote $W^{(L)}$ with initialized values (we have used the default initializer of pytorch). We need to ensure that forward propagation is done with sparse weights, so we modify $W_{\text{init}}^{(L)}$ to obtain the new initialized weight tensor for training as follows:


% Thereafter, in any epoch $t$, let $\nabla_{W^{(L)}_{t-1}}$ denote the gradient corresponding to $W^{(L)}_{t-1}$. Before making the gradient update (under optimizers like Adam, SGD, RMSProp), the gradient is modified as follows:


% The optimizer then uses the modified gradient for making the weight update.

% PAB: It is unclear you need dedicated hardware... Also, I'm not sure you want to make this the remark and emphasize your "trick" which appears to only require more FLOPs. I think Keith suggested the emphasis should be not on the trick but rather on the approach which explicitly avoids operating on zeros.
\subsection{FLOPs Count}

The FLOPs count for various CONV filter types are shown in Table \ref{tab:flops}.  This assumes a layer with IFM size of $H_i^L \times W_i^L \times C_i^L$ and OFM size $H_o^L \times W_o^L \times C_o^L$.   This is the  number of FLOPs required to perform the forward (i.e. inference) processing.  These expressions assume an efficient implementation as discussed above and are therefore ideal.  Specifically, the overhead with generating address and permutations -- i.e., in ShuffleNet and pSConv -- are not included in these expressions.  Note the the reduction in FLOPs for pSConv relative to the standard SFCC layer is  simply the kernel density -- \i.e. the KSS divided by the size of the standard 2D kernel.


\begin{table}[t]
  \centering
  \begin{tabular}{|c|c|}
  \hline
    Approach &  FLOP Count (Forward, Ideal) \\\hline \hline
    SFCC       & $H_o^L \times W_o^L \times C_i^L \times C_o^L \times k\times k$  \\\hline
    pSConv        & $ H_o^L \times W_o^L \times C_i^L \times C_o^L \times y $  \\\hline
    MobilNet-like     &   $(H_o^L \times W_o^L \times  C_i^L \times k \times k)$ \\
    (DWC-PWC) &  $+ (H_o^L \times W_o^L \times C_i^L \times C_o^L)$ \\\hline
    ShuffleNet-like    &  $(H_o^L \times W_o^L \times   C_i^L \times C_o^L \times k \times k)/G$  \\
    (GWC-DWC) & $+ (H_o^L \times W_o^L \times C_o^L \times k \times k)$ \\\hline
    \end{tabular}
  \caption{Expressions for the  FLOP count for the inference operations for various pre-defined constrained filter designs.}
  \label{tab:flops}
\end{table}


% In the following,  a layer $L$ is assumed to have an IFM size of $H_i^L \times W_i^L \times C_H^L$.
% FLOP count for a SFCC based CONV for this layer with $C$ filters, each of dimension mentioned in \ref{sub:psconv} to produce OFM of size $H_o^L \times W_o^L \times C$, is
% \begin{IEEEeqnarray}{c}\label{eq-flop1}
% FL_{SFCC} =  H_o^L \times W_o^L \times C_H^L \times C \times k\times k \IEEEyesnumber
% \end{IEEEeqnarray}
% For pSConv based CONV layer with $KS = y$ the FLOP count is
% \begin{IEEEeqnarray}{c}\label{eq-flop2}
% FL_{pSConv} =  H_o^L \times W_o^L \times C_H^L \times C \times y \IEEEyesnumber
% \end{IEEEeqnarray}
% A DWC+PWC layer for MobileNet-like architecture has the FLOP count of
% \begin{align}\label{eq-flop3}
% FL_{DP} = (H_o^L \times W_o^L \times & C_H^L \times k \times k) \nonumber\\
% &+ (H_o^L \times W_o^L \times C_H^L \times C)\IEEEyesnumber
% \end{align}
% Finally, a GWC+DWC layer implementation (ShuffleNet-like) with a group-size of G produces a FLOP count of
% \begin{align}\label{eq-flop4}
% FL_{GD} =  (H_o^L \times W_o^L \times & C_H^L \times C \times k \times k)/G \nonumber  \\
% & + (H_o^L \times W_o^L \times C \times k \times k)\IEEEyesnumber
% \end{align}
% Therefore, the reduction factor of FLOPs due to the replacement of SFCC with pSConv is given by
% \begin{align}\label{eq-flop5}
% R_{SFCC} =  &FL_{pSConv}/FL_{SFCC} = y/k^2 \IEEEyesnumber
% \end{align}
% Note the the reduction in (\ref{eq-flop5}) is simply the kernel densiity -- \i.e. the KSS divided by the size of the standard 2D kernel.

\begin{figure}[h!]
\includegraphics[width=0.9\linewidth]{Figs/pSC_conv_fig1.png}
\centering
\caption{pSConv: Proposed pre-defined sparse kernel based convolution with KSS of 4.}
\label{fig:pSConv}
\end{figure}



\iffalse
\begin{algorithm}[t]
\caption{Training pSConv for Conv2D Layer $l$ with Simple PyTorch Modifications (unoptimized)}  \label{algo:1}
\hspace*{\algorithmicindent} \textbf{Input:} $W_{\text{init}}^{(l)}$, $\alpha^{(l)}$ for Conv2D layer $l$, total training\\
\hspace*{\algorithmicindent} epochs $E$\\
% \hspace*{\algorithmicindent} worker $i$ \footnotemark  \\
\hspace*{\algorithmicindent} \textbf{Output:} Trained weight $W^{(l)}_E$ 
\begin{algorithmic}[1]
\Procedure{Initialization}{}
\State $W_0^{(l)} \gets \alpha^{(l)}\odot W_{\text{init}}^{(l)}$ 
\EndProcedure
\Procedure{Weight Update}{}

\For{$t \gets 1$ to $E$}                    
        \State Obtain $\nabla_{W^{(l)}_{t-1}}$ after backpropagation
        \State ${\nabla}_{W^{(l)}_{t-1}} \gets \alpha^{(l)} \odot \nabla_{W^{(l)}_{t-1}}$
        \State Obtain $\nabla_{W^{(l)}_{t}}$ using the optimizer
    \EndFor
\State \Return  $\nabla_{W^{(l)}_{E}}$
\EndProcedure
\end{algorithmic}
\end{algorithm}
\fi

\iffalse
\begin{figure}[htp]
\centering
\begin{subfigure}[t]{.45\textwidth}
\vspace{-.35cm}
\centering
\includegraphics[width=1\textwidth]{Figs/resnet18cifar10train.eps}
\caption{Training curves for ResNet-18 with varying degrees of sparsity.}
\vspace{.5cm}
\label{fig:sparseLenet5_train}
\end{subfigure}
~
\begin{subfigure}[t]{.45\textwidth}
\centering
  \includegraphics[width=1\textwidth]{Figs/resnet18cifar10val.eps}%
  \caption{Validation accuracy for ResNet-18 with varying degrees of sparsity.}
  \vspace{.5cm}
  \label{fig:sparseLenet5_test}
\end{subfigure}
\caption{Performance of pSConv for ResNet-18 on CIFAR-10.}
 \label{fig:resnet18cifar10}
\end{figure}
\fi


==> Allerton pSConv 2019/sec_results.tex <==

% In this section, we present experimental results to evaluate the pSConv method in various CNN-based architectures. We 
In this section we first give an overview of the experimental settings, and then discuss the results in detail for each experiment.
%\footnote{\textit{Pytorch} is used for all our neural network related operations.}
%% Pytorch has been stated in psconv section
\subsection{Datasets, Architectures, and Hyperparameters}
We use CIFAR-10 and Tiny ImageNet, two popular image classification datasets, for our evaluation. 
Both of these datasets comprise three-channel colored images.   CIFAR-10 has $10$ distinct classes, and each image  has a size of $(H_i^0,W_i^0,C_i^0) = (32, 32, 3)$, where $H_i^0$,$W_i^0$, and $C_i^0$ denote the input height, width, and number of channels, respectively. Tiny ImageNet has $200$ classes, and each image has a size of $(H_i^0,W_i^0,C_i^0) = (64,64,3)$. 


\begin{figure}[h!]
\includegraphics[width=0.8\linewidth]{Figs/shuffle_vs_pSConv.png}
\centering
\caption{A unit of (a) ShuffleNet bottleneck, (b) ResNet18 basic block, and (c) Modified ResNet18 with pSConv based basic block. }
\label{fig:Shuffle_vs_pSConv}
% PAB: You need to reference/describe this figure...
\end{figure}

We evaluate the benefits of pSConv on two state of the art neural network architectures -- ResNet18 \cite{he2016deep} and VGG16 \cite{simonyan2014very}. We defer the details of the architectures until the associated subsections that follow. For both ResNet18 and VGG16, we modified the level of sparsity in all of the $3 \times 3$ 2D kernels using the constrained, pseudo-random method described in Section \ref{sec:spCNN}, while the fully-connected and down-sampling layers are not modified. 

In each experiment, the number of training epochs is $60$. We use an initial learning rate of $0.1$ with a step decay of $0.2$ after $40^{th}$ and $55^{th}$ epoch. We use the stochastic gradient descent optimizer with a momentum of $0.9$ and weight decay of $0.0005$ for all experiments. A training dataset size of 40,000 with 10,000 each for validation and test is used for CIFAR-10 and training batch size is $128$. For Tiny ImageNet we use a training dataset of 100,000 images and 5000 images each for validation and test. The batch size for training is set to $100$. For each experiment, the final results have been presented for a single training experiment. In the following tables and figures, we denote the networks explored by the base network name, followed by the kernel support size  -- i.e., $\text{<basename>}\_\text{pSC<KSS>}$.  For example, ResNet$18\_\text{pSC4}$ denotes the ResNet18 architecture with $4$ non-zeros ($5$ zeros) in each 2D kernel. 

% Next we present the results from our experiments with ResNet18.
\iffalse
For both VGG16 and ResNet18, we evaluate the performance of our proposed pSConv approach by comparing the performance of the standard architecture with our architectures that have sparsity. Furthermore, as a baseline for comparing parameter and FLOP reduction, we use ShuffleNet, which is from the class of ShuffleNet neural networks that have recently become quite popular for neural network inference on edge devices \cite{wong2019attonets}. Our results demonstrate that state of the art architectures combined with pSConv can attain comparable FLOP and parameter count with much better accuracy than ShuffleNet. 
% PAB: I don't understand what you mean by "For this,"

%%%%%% Keith suggestion...
  The standard ResNet18 comprises a number of basic block computational layers, as shown in Fig.~\ref{fig:Shuffle_vs_pSConv}(b), along with down-sampling layers.  In all of our experiments, the down-sampling layers were not modified.  We modified the level of sparsity in all of the $3 \times 3$ 2D kernels using the constrained, pseudo-random method described in Section \ref{sec:spCNN}.  In order to more closely match the parameter count of ShuffleNet for various levels of sparsity, we introduced a modified version of ResNet18.  The standard of version of ResNet18 has computational layers that are groups of 4 of the basic blocks in Fig.~\ref{fig:Shuffle_vs_pSConv}(b).  The number of channels in the first layer of 4 blocks is 64 and increases to 128, 256, and 512, for the second, third, and fourth layer. Our modified version of ResNet18 uses half the number of channels in each of these layers (i.e., 32, 64, 128, 256).  We refer to this modified  ResNet18 as ``half-channel'' ResNet18 -- i.e., ResNet18$\_$HC.
\fi


\subsection{Experiments with ResNet18}
\begin{table*}[t]
  \centering
  \begin{tabular}{|c|c|c|c|c|c|}
  \hline
    Model & Test Acc $(\%)$ & FLOPs & FLOPs Reduced (\%) & Parameters & Parameters Reduced (\%) \\\hline
    ResNet18$\_$pSC9       & 91.3 & 0.559 G & ---& 11.17 M& --- \\\hline
    ResNet18$\_$pSC4       & \textbf{91.5} & 0.227 G & 59.4& 5.07 M&  54.6\\\hline
    ResNet18$\_$pSC2       & 90.8 & 0.117 G & 79.1& 2.63 M&  76.5\\\hline
    ResNet18$\_$HC$\_$pSC9 & 89.8 & 0.136 G & 75.7 & 2.8 M&  74.9\\\hline
    ResNet18$\_$HC$\_$pSC4 & 89.3 & 0.056 G & 89.9 & 1.27 M&  88.6\\\hline
    ResNet18$\_$HC$\_$pSC2 & 88.3 & \textbf{0.030 G} & \textbf{94.6}& \textbf{0.66 M} &  \textbf{94.1}\\\hline
    ShuffleNet          & 85.0 & 0.098 G & 82.5& 2.16 M&  80.7\\\hline
    \end{tabular}
  \caption{Performance evaluation of different variants of ResNet18 on CIFAR-10. The standard ResNet18 architecture is used as the reference for calculating the reduction in parameter and FLOP counts. In general, pSConv combined with the standard architectures can give significant improvements in FLOP and parameter counts with negligible drops in accuracy.}
  \label{tab:1}
\end{table*}

\begin{table*}[t]
  \centering
  \begin{tabular}{|c|c|c|c|c|c|}
  \hline
    Model &  Test Acc $(\%)$ & FLOPs & FLOPs Reduced (\%) & Parameters & Parameters Reduced (\%) \\\hline
    ResNet18$\_$pSC9   & \textbf{61.3} & 2.22 G & ---  &11.58 M & --- \\\hline
    ResNet18$\_$pSC4   & 60.7 & 0.902 G & 59.4 &5.47 M & 52.8 \\\hline
    ResNet18$\_$pSC2       & 59.4 & 0.463 G & 79.1 & 3.03 M& 73.8 \\\hline
    ResNet18$\_$HC$\_$pSC9 & 58.5 & 0.561 G & 74.7     & 3.00 M& 74.1 \\\hline
    ResNet18$\_$HC$\_$pSC4 & 57.3 & 0.228 G & 89.7     & 1.47 M& 87.3 \\\hline
    ResNet18$\_$HC$\_$pSC2 & 54.5 & \textbf{0.117 G} & \textbf{94.7}     & \textbf{0.863 M} & \textbf{92.6} \\\hline
    ShuffleNet          & 54.3 & 0.390 G & 82.4     & 3.37 M& 70.9 \\\hline
    \end{tabular}
  \caption{Performance evaluation of different variants of ResNet18 on Tiny ImageNet. The standard ResNet18 architecture is used as the reference for calculating the reduction in parameter and FLOP counts. In general, pSConv combined with the standard architectures   significant reduces the FLOP and parameter counts with negligible degradation in accuracy.}
  \label{tab:2}
\end{table*}


\iffalse
% PAB: This first sentence is repetitive with the overview subsection... Can't you just say "For our experiments with ResNet18 on CIFAR-10, we use"
We first present the results over CIFAR-10. We apply pSConv on each of the Conv2D layers, i.e. 17 layers. Furthermore, we consider the baseline ShuffleNet architecture, which as shown in Table \ref{tab:1}, has more than $80\%$ fewer parameters and FLOPs than the standard  ResNet18. To evaluate the benefits from pSConv, we modify the ResNet18 architecture such that the output channels in each of the Conv2D layers is reduced by a factor of $2$. This gives us the ResNet18$\_$HC, which has similar parameter and FLOP counts as ShuffleNet. Additionally, combining pSConv with ShuffleNet, we obtain fewer parameters and FLOPs.
\fi

In ResNet18, the first layer is a convolutional layer followed by batch normalization and ReLU. This is followed by $4$ layers each consisting of $2$ basic blocks. As illustrated in Fig. \ref{fig:Shuffle_vs_pSConv}(b), one basic block comprises  two paths for the input. The first path goes through a convolutional layer with $3\times 3$ kernel, followed by batch normalization and ReLU, which is followed by another convolutional layer with $3\times 3$ kernel and batch normalization. The second path is a skip connection, which is directly added to the result from the first path, and then passed through a ReLU. The skip connection path corresponding to the basic block which changes the input feature map dimension consists of $1 \times 1$ convolution layer with stride of 2 to match the dimension before adding. The output of the final basic block is flattened and fed into a fully connected layer with softmax, which has 10 output neurons for CIFAR-10 and $200$ output neurons for Tiny ImageNet. 

\begin{figure}[h!]
\includegraphics[width=0.8\linewidth]{Figs/fig1.png}
\centering
\caption{Validation accuracy vs epoch on CIFAR-10. The architectures being compared here are ShuffleNet, ResNet18$\_$HC$\_$pSC9 (standard ResNet18$\_$HC), and ResNet18$\_$HC$\_$pSC4 (ResNet18$\_$HC with 5 zeros (out of 9 elements) in each 2D kernel). }
\label{fig:fig1}
\end{figure}

\begin{figure}[!ht]
\includegraphics[width=0.8\linewidth]{Figs/ResNet18_CIFAR10_val_1.png}
\vspace*{-0.15in}
\centering
\newline
\caption{Validation accuracy vs epoch on CIFAR-10 for ResNet18$\_$pSC9 (standard architecture), ResNet18$\_$pSC4 (pSConv with $4$ non-zeros in each 2D kernel),  and ResNet18$\_$pSC2 (pSConv with $2$ non-zeros in each 2D kernel).}
\label{fig:fig2}
\end{figure}

 For standard ResNet18 the number of output channels in the first computational layer of 2 basic blocks is 64 and increases to 128, 256, and 512, for the second, third, and fourth computational layers, respectively. In order to more closely match the parameter count with ShuffleNet, we also use a modified version of ResNet18 with a channel width multiplier value of $0.5$. So, this modified version of ResNet18 uses half the number of channels in each of these computational layers (i.e., 32, 64, 128, 256). We refer to this modified  ResNet18 as ``half-channel'' ResNet18 -- i.e., ResNet18$\_$HC. For our work, we use a variant of ShuffleNet with group-size of 3 and channel depths of the stages as 384, 768 and 1536 which has comparable parameters count as ResNet18$\_$HC$\_$pSC9.

We first present our results on CIFAR-10. In Fig. \ref{fig:fig1}, we plot the validation accuracy vs epoch for ShuffleNet and ResNet18$\_$HC combined with pSConv. It shows both the ResNet18$\_$HC variants perform better at all the checkpoint epochs.  Also, it is clear from Table \ref{tab:1} that although ResNet18$\_$HC$\_$pSC4 (with only 4 non-zeros in each 2D kernel) and  ResNet18$\_$HC$\_$pSC2 (with only 2 non-zeros in each 2D kernel) have fewer parameters and FLOPs, they have significantly better test accuracy (89.3$\%$ and 88.3 $\%$, respectively) compared to ShuffleNet ($85.0\%$). 

In Fig. \ref{fig:fig2}, we plot validation accuracy vs epoch for the standard ResNet18, ResNet18$\_$HC and ResNet18 combined with pSConv. 
We see similar trend in validation accuracy improvement (including the jumps at epoch 40 and 55) for all the variants.

% PAB: This first sentence is also repetitive with the overview subsection, fix...
\begin{figure}[h!]
\includegraphics[width=0.8\linewidth]{Figs/fig4.png}
\centering
\caption{Validation accuracy vs epoch on Tiny ImageNet for ResNet18$\_$HC$\_$pSC9 (standard half-channel ResNet18), ResNet18$\_$HC$\_$pSC4 (pSConv with $4$ non-zeros in each 2D kernel),  and ResNet18$\_$HC$\_$pSC2 (pSConv with $2$ non-zeros in each 2D kernel).}
\label{fig:fig4}
\end{figure}

\begin{figure}[h!]
\includegraphics[width=0.8\linewidth]{Figs/ResNet18_Tiny_Image_val.png}
\vspace*{-0.15in}
\centering
\newline
\caption{Validation accuracy vs epoch on Tiny ImageNet for ResNet18$\_$pSC9 (standard architecture), ResNet18$\_$pSC4 (pSConv with $4$ non-zeros in each 2D kernel),  and ResNet18$\_$pSC2 (pSConv with $2$ non-zeros in each 2D kernel).}
\label{fig:fig5}
\end{figure}

Next we discuss our experimental results with Tiny ImageNet. In Fig. \ref{fig:fig4}, we plot the validation accuracy vs epoch for ShuffleNet and ResNet18$\_$HC combined with pSConv. Table \ref{tab:2} shows the comparison of FLOPs, parameter count and test accuracy. It is noteworthy that  ResNet18$\_$HC$\_$pSC2 (with only 2 non-zeros in each Conv2D kernel) with 3.3$\times$ lesser FLOP count provides similar accuracy as ShuffleNet.% PAB: differ more than VGG than what???}  (Table \ref{tab:2}), they have a faster convergence. Additionally, they have better test accuracy ($57.3\%$ and 54.5 $\%$) compared to ShuffleNet ($54.3\%$). These results are consistent with the results obtained for CIFAR-10. 


Fig. \ref{fig:fig5} illustrates the validation accuracy vs epoch for the standard ResNet18, ResNet18$\_$HC and ResNet18 combined with pSConv. Clearly, ResNet18$\_$pSC2 and  ResNet18$\_$pSC4 have similar validation accuracy improvement trend as the standard ResNet18, ResNet18$\_$HC. Furthermore, as illustrated in Table \ref{tab:2}, even for larger datasets pSConv can reduce the parameter and FLOP counts of the standard architectures without significant drop in test accuracy. 

\begin{figure}[h!]
\includegraphics[width=0.8\linewidth]{Figs/fig11.png}
\centering
\newline
\caption{Test accuracy vs parameter count for the experiments based on ResNet architectures. The results along the top correspond to CIFAR-10, while the results along the bottom correspond to Tiny ImageNet.}
\label{fig:fig11}
\end{figure}



Finally, in Fig. \ref{fig:fig11}, we plot the test accuracy as a function of parameter count for all the experiments related to ResNet18. For both CIFAR-10 and Tiny ImageNet, ResNet18$\_$HC$\_$pSC2 (half-channel ResNet18 with KSS of 2) has the lowest parameter count. With a 3.27$\times$ and 3.9$\times$ reduced parameter count compared to ShuffleNet, ResNet18$\_$HC$\_$pSC2 provides 3.3\% improved and similar accuracy on CIFAR-10 and Tiny ImageNet dataset, respectively. Furthermore, the parameters and FLOPs for ResNet18$\_$HC$\_$pSC9 and ResNet18$\_$pSC2 are quite similar, whereas the latter has around 1\% improved test accuracy for both the datasets.  This is somewhat in agreement with the trends observed in \cite{dey2019pre} for sparse multi-layer perceptrons (MLPs) where it was observed that using more neurons that are sparsely connected typically yields better performance than fewer neurons with full connectivity. Also somewhat surprisingly, the half-channel version of ResNet18 is an attractive, and simple, design alternative to ShuffleNet.


% Next we present the results with VGG16.


\subsection{Experiments with VGG16}

\begin{table*}[t]
  \centering
  \begin{tabular}{|c|c|c|c|c|c|}
  \hline
    Model & Test Acc $(\%)$ & FLOPs & FLOPs Reduced (\%) & Parameters & Parameters Reduced (\%) \\\hline
    VGG16$\_$pSC9       & 90.2 & 0.333 G & --- &33.65 M  & --- \\\hline
    VGG16$\_$pSC4       & 90.0 & 0.145 G & 56.5 &25.47 M & 24.3 \\\hline
    VGG16$\_$pSC2       & 88.8 & 0.082 G & 75.4 &22.20 M & 34.0 \\\hline
    \end{tabular}
  \caption{Performance evaluation of different variants of VGG16 on CIFAR-10. Applying pSConv results in a parameter reduction of up to $34.0\%$ and FLOP count reduction by up to $75.4 \%$.}
  \label{tab:3}
\end{table*}

% PAB: This first sentence is also repetitive with the overview subsection. Perhaps just remove it.. and start next sentence as "In VGG16, there are.....

In VGG16, there are $13$ convolutional layers, where each convolutional layer is followed by batch normalization and ReLU. There are max pooling layers after ReLU corresponding to the convolutional layers $2$, $4$, $7$, $10$ and $13$. The last max pooling layer feeds an average pooling layer. The next two layers are fully connected layers with ReLUs, while the final layer is a fully connected layer with softmax having 10 output neurons for CIFAR-10 and $200$ output neurons for Tiny ImageNet. 

\begin{figure}[!ht]
\includegraphics[width=0.8\linewidth]{Figs/VGG16_CIFAR10_val.png}
\vspace*{-0.15in}
\centering
\newline
\caption{Validation accuracy vs epoch on CIFAR-10 for VGG16$\_$pSC9 (standard architecture), VGG16$\_$pSC4 (pSConv with $4$ non-zeros in each 2D kernel),  and VGG16$\_$pSC2 (pSConv with $2$ non-zeros in each 2D kernel).}
\label{fig:fig8}
\end{figure}

For VGG16 with CIFAR-10, we summarize the results in Table \ref{tab:3}, where we can clearly see that with a decrease in KSS, both parameter and FLOPs decrease significantly, with a modest decrease in test accuracy. As illustrated by Fig.\ref{fig:fig8}, architectures with pSConv have a similar convergence curve for validation accuracy as that of the standard architecture. 

\begin{table*}[t]
  \centering
  \begin{tabular}{|c|c|c|c|c|c|}
  \hline
    Model & Test Acc $(\%)$ & FLOPs & FLOPs Reduced (\%) & Parameters & Parameters Reduced (\%) \\\hline
    VGG16$\_$pSC9       &  54.2 &  1.28 G & --- & 40.72 M  & --- \\\hline
    VGG16$\_$pSC4       &  53.5 &  0.528 G & 58.8 & 32.54 M & 20.1 \\\hline
    VGG16$\_$pSC2       &  51.8 &  0.277 G & 78.4 & 29.28 M & 28.1 \\\hline
    \end{tabular}
  \caption{Performance evaluation of different variants of VGG16 on Tiny ImageNet. Applying pSConv results in a parameter reduction of up to $28.1\%$ and FLOP count reduction by up to $78.4 \%$.}
  \label{tab:4}
\end{table*}

\begin{figure}[!ht]
\includegraphics[width=0.8\linewidth]{Figs/VGG16_Tiny_image_val.png}
\vspace*{-0.15in}
\centering
\newline
\caption{Validation accuracy vs epoch on Tiny ImageNet for VGG16$\_$pSC9 (standard architecture), VGG16$\_$pSC4 (pSConv with $4$ non-zeros in each 2D kernel),  and VGG16$\_$pSC2 (pSConv with $2$ non-zeros in each 2D kernel).}
\label{fig:fig9}
\end{figure}

% PAB: Again, avoid the redundancy here...
Similar results are obtained for training over Tiny ImageNet. As shown in Table \ref{tab:4}, as KSS is decreased, both parameter and FLOPs count decrease significantly, with only a modest decrease in test accuracy. Specifically, we see a reduction of parameter and FLOPs count by $28.1\%$ and $78.4\%$, respectively.\footnote{VGG has a larger portion of its parameters  in the fully-connected classification layers than ResNet18, so the FLOPs reduction and parameter count reductions differ less for VGG than for ResNet18.} Furthermore, as illustrated by Fig. \ref{fig:fig9}, architectures with pSConv have a similar convergence curve for validation accuracy as that of the standard architecture. 

\iffalse
our experimental results for different architectures with varying values of $\alpha$. The following two cases are considered for the experiments:

\begin{itemize}
    \item \textbf{Case A}: In the first case, we use the MNIST dataset and LeNet5 architecture and vary sparsity using $\alpha\in\{0,0.4,0.6,0.8\}$.
    \item \textbf{Case B}: In the second case, we use the CIFAR-10 dataset and ResNet18 architecture and vary sparsity using $\alpha\in\{0,0.6,0.8,0.9\}$.
\end{itemize}
The training and inference curves for cases A and B have been presented in Fig. \ref{fig:sparseCNN_LeNet5} and Fig. \ref{fig:sparseCNN_ResNet18} respectively.



\iffalse
\begin{figure}[htp]
\centering
\begin{subfigure}[t]{.45\textwidth}
\vspace{-.35cm}
\centering
\includegraphics[width=1.0\textwidth]{Figs/ResNet18_sparse_train}
\caption{Training curves for ResNet18 with varying degrees of sparsity.}
\vspace{.5cm}
\label{fig:sparseResNet18_train}
\end{subfigure}
~
\begin{subfigure}[t]{.45\textwidth}
\centering
  \includegraphics[width=0.8\textwidth]{Figs/ResNet18_sparse_test}%
  \caption{Test accuracy after training for $60$ epochs for ResNet18 with varying degrees of sparsity.}
  \vspace{.5cm}
  \label{fig:sparseResNet18_test}
\end{subfigure}
\caption{Training and inference results for Case B. Adam optimizer is used.}
 \label{fig:sparseCNN_ResNet18}
\end{figure}

\fi
We summarize our observations below:

\begin{itemize}
    \item Introducing pseudo-random sparsity in convolutional layers is a promising method for reducing parameters in convolutional layers.
    \item As demonstrated by Fig. \ref{fig:sparseLenet5_test} and Fig. \ref{fig:sparseResNet18_test}, having sparsity may give faster convergence in test accuracy in comparison to the network without any pre-defined sparsity.
    \item With convolutional layers forming a major component in the modern neural network architectures, one can get significant reduction in parameters by sparsity in convolutional layers. This is demonstrated by Table \ref{tab:sparseCNN_ResNet18}.
    
\end{itemize}

\begin{table}[htp]
\begin{center}
\caption{Overall reduction in trainable parameter count for different sparsity for Case B.}
\label{tab:sparseCNN_ResNet18}
\begin{tabular}{|c|c|c|}
\hline
Sparsity & Trainable &  Parameter 	 \\ 
  & parameters  &  Reduction factor	 \\ \hline
$0.0$ & $11173962$  & $1\times$	 \\ \hline
$0.6$ & $5060352$   & $\sim 2.1\times$	\\ \hline
$0.8$ & $2618752$ & $\sim 4.1\times$	\\ \hline
$0.9$ & $1397952$ & $\sim 8\times$	\\ \hline
\end{tabular}
\end{center}
\end{table}

\fi

% PAB: Consider adding a discussion or summary subsection... that includes the new figure...

